\textsc{Perseus}: Tracing the Masterminds Behind Cryptocurrency Pump-and-Dump Schemes

Masterminds are entities organizing, coordinating, and orchestrating cryptocurrency pump-and-dump schemes, a form of trade-based manipulation undermining market integrity and causing financial losses for unwitting investors. Previous research detects pump-and-dump activities in the market, predicts the target cryptocurrency, and examines investors and \ac{osn} entities. However, these solutions do not address the root cause of the problem. There is a critical gap in identifying and tracing the masterminds involved in these schemes. In this research, we develop a detection system \textsc{Perseus}, which collects real-time data from the \acs{osn} and cryptocurrency markets. \textsc{Perseus} then constructs temporal attributed graphs that preserve the direction of information diffusion and the structure of the community while leveraging \ac{gnn} to identify the masterminds behind pump-and-dump activities. Our design of \textsc{Perseus} leads to higher F1 scores and precision than the \ac{sota} fraud detection method, achieving fast training and inferring speeds. Deployed in the real world from February 16 to October 9 2024, \textsc{Perseus} successfully detects $438$ masterminds who are efficient in the pump-and-dump information diffusion networks. \textsc{Perseus} provides regulators with an explanation of the risks of masterminds and oversight capabilities to mitigate the pump-and-dump schemes of cryptocurrency.

==> new_section/threat_model.tex <==
\section{Formalization of Problem}

\subsection{Problem Formalization}


Let $V$ represent the set of spreaders partitioned into masterminds $V_m$ and accomplices $V_n$, such that $V = V_m \cup V_n$. Define $V_m$ as the set of masterminds $\{v_{m_1}, v_{m_2}, \dots, v_{m_i}\}$ and $V_n$ as the set of accomplices $\{v_{n_1}, v_{n_2}, \dots, v_{n_j}\}$. The spreaders utilize \acs{osn}s to propagate crowd-pumps messages, forming information diffusion pathways as edges $E$ in a graph $G$. Thus, the graph $G = (V, E)$ defines the crowd-pump information diffusion network.

A crowd-pump labeled $c$ includes detailed messages specifying the target cryptocurrency $x$ and price levels for buying and selling the coin. Each crowd-pump left marks of message timing $t$, spreader identity $v$. Once a crowd-pump message is sent on a Telegram channel, other spreaders read and rebroadcast it, passing on the information. We refer to this process of crowd-pump information diffusion as a crowd-pump event $d$. Thus, over a period of time $T$, a crowd-pump event $d$ targeting cryptocurrency $x$ can be formalized as $d^x_T =  \{(c_1), (c_2), \ldots, (c_n)\}$.
For a specific cryptocurrency over the union of periods $\tau$, where $\tau = T_1 \cup T_2 \cup \ldots \cup T_n$, we observe an array of crowd-pump events, $D^x_\tau$, which can be formalized as $D^x_\tau = \{d^x_{T_1},d^x_{T_2}, \ldots, d^x_{T_n} \}.$



\textsc{Perseus}'s task is to infer the edges $E$ from patterns of information diffusion $D^x_\tau$ to construct the crowd-pump spreader network $G$ and classify the spreaders $V$ into the masterminds $V_m$ and the accomplices $V_n$.


\subsection{Threat Model}
\input{exhibits/new/comparisons}

Due to the avoidance of precise timing coordination, crowd-pumps are more prevalent than time-pumps, as depicted in \autoref{fig:comparison}, posing significant economic threats. Thus, we design \textsc{Perseus} based on the characteristics of crowd-pump information diffusion to detect masterminds. Masterminds disseminate crowd-pump messages across \acs{osn}s to impact the cryptocurrency market, in which we observe market price fluctuations from the cryptocurrency market and crowd-pump messages from \acs{osn}s. To avoid the detection system, masterminds can utilize the following strategy.  

($i$) Edge manipulation. Masterminds can coordinate with accomplices to broadcast the crowd-pump messages simultaneously. In this way, masterminds introduce $E_{concurrent}$'s into $E$, which may not represent the real structure of the crowd-pump spreader network graph $G$. 


($ii$) Node addition. Masterminds can create channels not within our investigation scope, introducing a new node, $v_{new}$, into $V$. In this way, masterminds change the topological features of the graph $G$.


($iii$) Identity manipulation. Masterminds can utilize bots to disseminate crowd-pump messages, introducing disguised node $V_{bot}$ into $V$. By doing this, masterminds can hide their identity without revealing the account metadata.  

==> slides/background.tex <==
% \begin{frame}{Background: }
%     \begin{multicols}{2} 
%         \begin{enumerate}
%             % \item Individuals or groups purchase a cryptocurrency, artificially inflate its price through strategic trading and subsequently sell it at a profit. Importantly, all illicit pump activities include a dump phase.
%             \item Pump-and-dump schemes depend on coordinated buying and selling of targeted cryptocurrencies. 
%             \item Time-pumps rely on precise synchronization of buying and selling activities on exchanges across multiple OSN.
%             \item crowd-pumps are organized through predefined price boundaries across OSNs, coordinating participants to execute trades on exchanges accordingly.
%         \end{enumerate} 

%         \columnbreak
%         % \begin{figure}
%         %     \centering
%         %     \includegraphics[width=\linewidth]{img/new/}

%         % \end{figure}
%         \input{exhibits/new/comparisons}
%     \end{multicols}
% \end{frame}



% \begin{frame}{Background: }
%     \begin{multicols}{2} 
%         \begin{enumerate}
%             \item OSNs are exploited by spreaders to enhance the effects of crowd-pumps.
%             \item Spreaders establish channels where only they can talk to coordinate investors to trade with the crowd-pump messages.
%             \item Masterminds initiate these crowd-pump messages.
%             \item Community: Accomplices of the masterminds further propagate them.
%             \item Information diffusion (Crowd-pump event): crowd-pump messages flow from masterminds to their accomplices.
%         \end{enumerate} 

%         \columnbreak
%         % \begin{figure}
%         %     \centering
%         %     \includegraphics[width=\linewidth]{img/new/}

%         % \end{figure}
%         \input{exhibits/new/POWR}
%     \end{multicols}
% \end{frame}



% \begin{frame}{Problem Formalization}
% \begin{enumerate}
%     \item Let $V$ represent the set of spreaders partitioned into masterminds $V_m$ and accomplices $V_n$, such that $V = V_m \cup V_n$. Define $V_m$ as the set of masterminds $\{v_{m_1}, v_{m_2}, \dots, v_{m_i}\}$ and $V_n$ as the set of accomplices $\{v_{n_1}, v_{n_2}, \dots, v_{n_j}\}$.
%     \item The spreaders utilize OSNs to propagate crowd-pumps messages, forming information diffusion pathways as edges $E$ in a crowd-pump information diffusion graph $G$. 
%     % \item The graph $G = (V, E)$ defines the crowd-pump information diffusion network.
%     \item A crowd-pump labeled as $c$ includes the target cryptocurrency $x$. Each crowd-pump left a mark of message timing $t$ and spreader identity $v$.
%     \item Crowd-pump information diffusion is a crowd-pump event $d$. Over time $T$, a crowd-pump event $d$ targeting cryptocurrency $x$ is formalized as $d^x_T =  \{(c_1), (c_2), \ldots, (c_n)\}$.
%     \item Over the union of periods $\tau$, where $\tau = T_1 \cup T_2 \cup \ldots \cup T_n$, we observe an array of crowd-pump events, $D^x_\tau$, where $D^x_\tau = \{d^x_{T_1},d^x_{T_2}, \ldots, d^x_{T_n} \}.$
%     \item Perseus infers the edges $E$ from patterns of information diffusion $D^x_\tau$ to construct the network $G$ and classify the spreader of $V$ into the masterminds $V_m$ and the accomplices $V_n$.

% \end{enumerate}

% \end{frame}


\begin{frame}{System Design}
\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{img/new/pipeline.pdf}
  \caption{The proposed mastermind detection system consists of three components: real-time fetcher, temporal attributed graph generator, and mastermind detector. Both data extraction and data processing operate concurrently to analyze data from OSNs and cryptocurrency markets.}
  \label{fig:pipeline}
\end{figure}

\end{frame}



% \begin{frame}{System Design}
% Real-Time Fetcher
% \begin{itemize}
%     \item OSN platform
%     \begin{enumerate}
%     \item Identify relevant Telegram channels using the search terms crypto pump Telegram and crypto signal Telegram in search engines Google and Bing. 
%     \item Deploy automated bots to scrape real-time raw text messages from each channel, capturing invitation links to additional Telegram channels. 
%     \item Follow these invitation links, we expand our list of channels.
%     \item The bots scrape metadata from each channel, including the timestamp $t$ of each message and the channel identifiers $v$'s.
%     \end{enumerate}
%     \item Crypto market
%     \begin{enumerate}
%         \item For each cryptocurrency $x$, we fetch transactions covering three days before and after each crowd-pump message, including detailed minute-by-minute and trade-by-trade price information for each targeted cryptocurrency. 
%         % \item We choose three days as the window size because the reported duration from the crowd-pump messages usually will not exceed three days. 
%         \item Given the substantial volume of trades with Ethereum (ETH) and Bitcoin (BTC), we capture data at one-minute intervals to reflect market responses to each crowd-pump. 
%     \end{enumerate}
% \end{itemize}
% \end{frame}




% \begin{frame}{System Design}
% Temporal Attributed Graph Generator
% \begin{enumerate}
%     \item OSN processing
%     \begin{itemize}
%     \item Named Entity Recognition: we extract named entities such as the names of cryptocurrencies, associated target prices, and advised trading positions (long or short).
%     \item OSN Feature: \textbf{total number of crowd-pump messages}.
%     \item Crowd-pump Event Establishment: we select a time period, $\tau$, and group the crowd-pump messages by the same cryptocurrency and the same direction of the trade. We divide each message group into separate crowd-pump events using a specific time gap threshold. 
%     \item Graph Construction
%     \item Topological Features: \textbf{out nodes, clustering coefficient, closeness centrality, betweenness centrality, PageRank, Density, Effective size, efficiency, out-ratio } ,and \textbf{in-ratio}.

%     \end{itemize}

%     \item Crypto market processing
%     \begin{itemize}
%         \item To measure the impact of each crowd pump message, we calculate the maximum return within a three-day window post-announcement.  
%         \item Market features: \textbf{Average Increase Percentages}, \textbf{Total Targets Achieved}, and \textbf{Rating}.
%     \end{itemize}
% \end{enumerate}
    
% \end{frame}






% \begin{frame}{Graph Construction}
% By adapting the proof of DANI (Diffusion Aware Network Inference Algorithm), we prove that\[
% G' \propto \underset{G}{\mathrm{argmax}} \left( \sum_{(r,s) \in G} \sum_{d_i \in D^x_\tau} \left(\frac{\theta_{rs}}{\lambda^{(i)}_{rs}} \right) \right).\]
% Thus, we compute the adjacent matrix by maximizing the likelihood of the above:
% \[G' = \underset{G | 0 \leq W \leq 1}{\mathrm{argmax}}\ P(D^x_\tau|G),\] where $W=\frac{\theta_{rs}}{\lambda_{rs}}$ is a weighted adjacent matrix. $\theta_{rs} = \frac{|\mathcal{I}_n(r) \cap \mathcal{I}_n(s)|}{|\mathcal{I}_n(r) \cup \mathcal{I}_n(s)|}$ and 
% $\lambda^{(i)}_{rs} = \frac{h^{(i)}_{rs}}{\sum_{y \in V_{D^{x}_{\tau}
% }} h^{(i)}_{ry}}$ are two parameters used for preserving the community structure and directionality of information diffusion. 
% \end{frame}

\begin{frame}{Graph Construction}
    \begin{multicols}{2} 


    
$ G' \propto \underset{G}{\mathrm{argmax}} \left( \sum_{(r,s) \in G} \sum_{d_i \in D^x_\tau} \left(\frac{\theta_{rs}}{\lambda^{(i)}_{rs}} \right) \right)$$

$G' = \underset{G | 0 \leq W \leq 1}{\mathrm{argmax}}\ P(D^x_\tau|G)$ 

$W=\frac{\theta_{rs}}{\lambda_{rs}}$ is a weighted adjacent matrix. 

$\theta_{rs} = \frac{|\mathcal{I}_n(r) \cap \mathcal{I}_n(s)|}{|\mathcal{I}_n(r) \cup \mathcal{I}_n(s)|}$ and 
$\lambda^{(i)}_{rs} = \frac{h^{(i)}_{rs}}{\sum_{y \in V_{D^{x}_{\tau}
}} h^{(i)}_{ry}}$ are two parameters used for preserving the community structure and directionality of information diffusion. 


        \columnbreak

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.85\linewidth]{img/new/DANI.pdf}
  \caption{Example of graph inference steps.}
  \label{fig:graph_infer}
\end{figure}
    \end{multicols}

\end{frame}



% \begin{frame}{Graph Construction}
%      In step I, we compute the announcement time ranking vector, which involves sorting the announcement times to derive the ranking vector of the spreaders. For instance, in the case of event \(d_1\), the corresponding ranking vector is \(l^1 = \begin{bmatrix}M & A & B\end{bmatrix}\), which indicates the order in which the spreaders broadcast the information. In step 2, we calculate the information directionality parameter, specifically \(h\) and \(\lambda\). For example, the calculation of \(h^{(1)}_{MA}\) is given by:
%     \[
%     h^{(1)}_{MA} = \frac{1}{ l^{(1)}_{A} \times (l^{(1)}_{A} - l^{(1)}_{M})} = \frac{1}{2 \times (2 - 1)}
%     \]
%     Here, the index \(2\) corresponds to spreader \(A\), and the index \(1\) corresponds to spreader \(M\) in the ranking vector \(l^1\). Subsequently, \(\lambda^{(1)}_{MA}\) is computed as:
%     \[
%     \lambda^{(1)}_{MA} = \frac{h^{(1)}_{MA}}{ h^{(1)}_{MA} + h^{(1)}_{MB}}
%     \]
%     This calculation is based on the fact that spreader \(M\) has two outward edges, specifically \(\lambda^{(1)}_{MA}\) and \(\lambda^{(1)}_{MB}\). In step 3, we determine the community structure parameter by computing \(\bm{\mathcal{I}_n}\) and \(\theta\). For example, \(\mathcal{I}_n(M) = \{d_1, d_3\}\) and \(\mathcal{I}_n(A) = \{d_1, d_2, d_3\}\) represent the sets of crowd-pump events in which spreaders \(M\) and \(A\) participate, respectively. The community structure parameter \(\theta_{MA}\) is calculated as:
%     \[
%     \theta_{MA} = \frac{|\mathcal{I}_n(M) \cap \mathcal{I}_n(A)|}{|\mathcal{I}_n(M) \cup \mathcal{I}_n(A)|}
%     \]
%     Here, the size of the intersection of the two sets is divided by the size of their union. In step 4, we combine the information directionality and community structure parameters across all crowd-pump events to construct the information diffusion graph. In this specific case, the edge \(e_1\) is given by:
%     \[
%     w_{MA} = \theta_{MA} \times \frac{\lambda^{(1)}_{MA} + \lambda^{(3)}_{MA}}{\lambda^{(1)}_{MA} + \lambda^{(3)}_{MA} + \lambda^{(1)}_{MB}}
%     \]
%     This incorporates both the directionality and community structure parameters across all crowd-pump events to represent the diffusion of information within the network.
% \end{frame}


% \begin{frame}{Graph Construction}
%  In step I, we compute the announcement time ranking vector, which involves sorting the announcement times to derive the ranking vector of the spreaders. For instance, in the case of event \(d_1\), the corresponding ranking vector is \(l^1 = \begin{bmatrix}M & A & B\end{bmatrix}\), which indicates the order in which the spreaders broadcast the information. In step 2, we calculate the information directionality parameter, specifically \(h\) and \(\lambda\). For example, the calculation of \(h^{(1)}_{MA}\) is given by:
%     \[
%     h^{(1)}_{MA} = \frac{1}{ l^{(1)}_{A} \times (l^{(1)}_{A} - l^{(1)}_{M})} = \frac{1}{2 \times (2 - 1)}
%     \]
%     Here, the index \(2\) corresponds to spreader \(A\), and the index \(1\) corresponds to spreader \(M\) in the ranking vector \(l^1\). Subsequently, \(\lambda^{(1)}_{MA}\) is computed as:
%     \[
%     \lambda^{(1)}_{MA} = \frac{h^{(1)}_{MA}}{ h^{(1)}_{MA} + h^{(1)}_{MB}}
%     \]
%     This calculation is based on the fact that spreader \(M\) has two outward edges, specifically \(\lambda^{(1)}_{MA}\) and \(\lambda^{(1)}_{MB}\). In step 3, we determine the community structure parameter by computing \(\bm{\mathcal{I}_n}\) and \(\theta\). For example, \(\mathcal{I}_n(M) = \{d_1, d_3\}\) and \(\mathcal{I}_n(A) = \{d_1, d_2, d_3\}\) represent the sets of crowd-pump events in which spreaders \(M\) and \(A\) participate, respectively. The community structure parameter \(\theta_{MA}\) is calculated as:
%     \[
%     \theta_{MA} = \frac{|\mathcal{I}_n(M) \cap \mathcal{I}_n(A)|}{|\mathcal{I}_n(M) \cup \mathcal{I}_n(A)|}
%     \]
%     Here, the size of the intersection of the two sets is divided by the size of their union. In step 4, we combine the information directionality and community structure parameters across all crowd-pump events to construct the information diffusion graph. In this specific case, the edge \(e_1\) is given by:
%     \[
%     w_{MA} = \theta_{MA} \times \frac{\lambda^{(1)}_{MA} + \lambda^{(3)}_{MA}}{\lambda^{(1)}_{MA} + \lambda^{(3)}_{MA} + \lambda^{(1)}_{MB}}
%     \]
%     This incorporates both the directionality and community structure parameters across all crowd-pump events to represent the diffusion of information within the network.
    
% \end{frame}

% \begin{frame}{Directed vs weighted information diffusion}
% % $w_{rs}=\frac{\theta_{rs}}{\lambda_{rs}}$ is a critical. It is derived from aggregating diffusion information probability matrix $\lambda$ with community structure preserving matrix $\theta$. For each pair of node \( (r, s )\) in $G_{D^x_\tau}$, we construct two set of embedding, weighted DANI and directed DANI. The weighted DANI embedding is just the adjacent matrix $w_{rs}$, but directed DANI embedding $w*_{rs}$ is created as follows:
% \begin{equation}
%     w*_{rs} = 
%     \begin{cases} 
%         1 & \text{if } w_{rs} > w_{sr} \\
%         0 & \text{otherwise.}
%     \end{cases}
% \end{equation}

% \begin{figure}[!t]
%     \centering
%     % First mini-page for the first plot
%     \begin{minipage}{0.15\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{img/new/embedding1.pdf}
%         \subcaption{}
%         \label{subfig:wd}
%     \end{minipage}
%     \begin{minipage}{0.15\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{img/new/embedding2.pdf} 
%         \subcaption{}
%         \label{subfig:dd}

%     \end{minipage}
%     \caption{Nodes represent spreaders. (a) corresponds to weighted diffusion graphs, in which wider edges correspond to higher likelihood of information passing. Edges may also be reciprocal. (b) corresponds to the directed diffusion graphs, in which edges are directed and not reciprocal.}
%     \label{fig:directedvsweighted}

% \end{figure}

% \end{frame}


% \begin{frame}{Topological Features}
% We include traditional topological features such as \textbf{clustering coefficient, closeness centrality, betweenness centrality,} and \textbf{PageRank} 

% \input{tables/unweighted_features}

% \end{frame}



% \begin{frame}{Mastermind Detection}
% \begin{itemize}
%     \item For each graph $G_{D^x_\tau}=(E(D^x_\tau), V(D^x_\tau))$, we assume that at least one node, $v_m \in V(D^x_\tau)$, represents a mastermind organizing the crowd-pump events. Each node $v_i \in V(D^x_\tau)$ is associated with a feature vector $\mathbf{x}_i \in \mathbb{R}^n$. Given the labels $\{y_i\}_{i=1}^{|V|}$, where $y_i$ represents the label of node $v_i$, Perseus' objective is to learn a mapping function $f: \mathbb{R}^d \rightarrow \mathbb{R}$ that assigns a probability score to each node, representing how likely it is to be a mastermind. 

%     \item To achieve this, we apply GAT and GraphSAGE to distinguish masterminds from accomplices. These architectures are combined with the temporal attributed graphs, offering distinct approaches to aggregating information from neighboring nodes.
% \end{itemize}


% \end{frame}


% \begin{frame}{Mastermind Detection: Temporal and non-temporal tasks}
%     \begin{multicols}{2} 
%         Temporal and non-temporal tasks datasets. The dataset is divided chronologically into training, validation, and testing segments for temporal tasks. Specifically, training is conducted on the earliest data, validation on subsequent data, and testing on the most recent data. In contrast, for non-temporal tasks, the data selection process is randomized. 70\% of the graphs from three distinct periods are selected for training, while 15\% are allocated for validation and another 15\% for testing.

%         \columnbreak
%         \begin{figure}
%             \centering
%             \includegraphics[width=\linewidth]{img/new/temporal.pdf}

%         \end{figure}
%     \end{multicols}
% \end{frame}


\begin{frame}{Evaluation: Accuracy}


  \begin{columns}[c]
    \begin{column}{0.32\textwidth}
      \centering
      \includegraphics[width=\linewidth]{img/new/jan_precision_plot.pdf}
      \small (a) Precision
      \label{fig:precision}
    \end{column}
    \begin{column}{0.32\textwidth}
      \centering
      \includegraphics[width=\linewidth]{img/new/jan_f1_plot.pdf}
      \small (b) F1 Score
      \label{fig:f1}
    \end{column}
    \begin{column}{0.32\textwidth}
      \centering
      \includegraphics[width=\linewidth]{img/new/jan_combined_roc_plot.pdf}
      \small (c) AUC
      \label{fig:auc}
    \end{column}
  \end{columns}

  \vspace{0.5cm}

  \small
  Figure (a) shows the precision of four models varying thresholds. Figure (b) shows the F1 of four models varying thresholds. Figure (c) shows the AUC of four models varying thresholds.


\end{frame}


% \begin{frame}{Evaluation: Mastermind Labelling}
% \begin{table}[!h]
% \centering
% \tiny
% \caption{Crowd-pump Messages and Returns}
% \label{tab:case_study}
% \begin{tabularx}{\textwidth}{|c|l|c|X|c|}
% \hline
% \textbf{Events} & \textbf{Telegram Channels} & \textbf{Timestamps} & \textbf{Messages} & \textbf{Returns} \\ 
% \hline
% \textcolor{red}{d1} & \textcolor{red}{bitcoinpumpgroup} & \textcolor{red}{2021-01-12 06:11:41} & \textcolor{red}{\#NEBL (Binance) Buy Range : 1450-1600 Target 1: 1750 Target 2: 1900 Target 3: 2100 Stop loss: 1300} & \textcolor{red}{22.44\%} \\
%    & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{2021-01-14 17:55:30} & \textcolor{red}{\#NEBL (Binance) Buy zone 2100-2200 Sell zone 2308-2424-2655-3001+ By @crypto\_pump\_island (@APGLOBALS)} &\textcolor{red}{25.30\%} \\
% \hline
% \textcolor{red}{d2} & \textcolor{red}{bitcoinpumpgroup} & \textcolor{red}{2021-02-07 03:36:15} & \textcolor{red}{\#NEBL (Binance) Buy Range : 2754 - 3240 Target 1: 3531 Target 2: 3823 Target 3: 4212 Stop loss: 2430 Contact  @bitcoinadmin  for VIP membership} & \textcolor{red}{8.72\%} \\
%    & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{2021-02-07 03:59:16} & \textcolor{red}{\#NEBL (Binance) Buy zone 3000-3220 Sell zone 3400-3767-4126-4664+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{16.89\%} \\
% \hline
% \textcolor{red}{d3} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{2021-02-11 05:01:44} & \textcolor{red}{\#NEBL (Binance) Buy zone 3550-3850 Sell zone 4043-4246-4650-5256+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{36.46\%} \\
%    & \textcolor{red}{bitcoinpumpgroup} & \textcolor{red}{2021-02-11 05:01:44} & \textcolor{red}{\#NEBL (Binance) Buy Range : 2754 - 3240 Target 1: 3531 Target 2: 3823 Target 3: 4212 Stop loss: 2430} & \textcolor{red}{1.40\%} \\
% \hline
% \textcolor{red}{d4} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{2021-04-11 07:20:08} & \textcolor{red}{\#NEBL (Binance) Buy zone 6000-6650 Sell zone 6900-7213-7900-8930+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{12.00\%} \\
%    & mega\_pump\_signals & 2021-04-11 07:20:29 & \#NEBL (Binance) Buy zone 6000-6650 Sell zone 6900-7213-7900-8930+ By @crypto\_pump\_island (@APGLOBALS) & 12.24\% \\
%    & BinanceSuperPumpSignals & 2021-04-11 09:04:34 & \#NEBL (Binance) Buy zone 6566-7060 Sell zone 7403-7889-8666-14567 & 17.64\% \\
% \hline
% \textcolor{red}{d5} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{2021-06-13 09:33:20} & \textcolor{red}{\#NEBL (Binance) Buy zone 5800-6240 Sell zone 6592-6922-7581-8570+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{0.32\%} \\
%    & mega\_pump\_signals & 2021-06-13 09:33:37 & \#NEBL (Binance) Buy zone 5800-6240 Sell zone 6592-6922-7581-8570+ By @crypto\_pump\_island (@APGLOBALS) & 0.32\% \\
% \hline
% \textcolor{red}{d6} & \textcolor{red}{bitcoinpumpgroup} & \textcolor{red}{2022-11-22 16:59:09} & \textcolor{red}{\#NEBL (Binance) Buy Range : 9785 - 11512 Target 1: 12432 Target 2: 13238 Target 3: 15080 Stop loss: 8634} & \textcolor{red}{24.19\%} \\
%    & crypto\_pump\_lsIand& 2022-11-24 21:18:08 & Buy zone 10342-11232 Sell zone 11676-12677-13456-14901+ By @crypto\_pump\_island (@APGLOBALS) & 18.62\% \\
% \hline
% \textcolor{red}{d7} & \textcolor{red}{bitcoinpumpgroup} & \textcolor{red}{2023-02-09 14:55:00} & \textcolor{red}{\#NEBL (Binance) Buy Range : 6290 - 7400 Target 1: 7992 Target 2: 8510 Target 3: 9694 Stop loss: 5550} & \textcolor{red}{6.95\%} \\
%    & backstreetbets & 2023-02-09 14:56:54 & \#NEBL (Binance) Buy Range : 6290 - 7400 Target 1: 7992 Target 2: 8510 Target 3: 9694 Stop loss: 5550 & 7.22\% \\
% \hline

% \end{tabularx}
% \end{table}


% \end{frame}




\begin{frame}{Evaluation: Training and Inferring Speed}
\input{exhibits/new/auc_training}
 
\end{frame}



\begin{frame}{Evaluation: Benchmark Comparison}
\input{tables/mastermind}
 
\end{frame}




% \begin{frame}{Evaluation: Mastermind Detection}
% \input{tables/mastermind_updated}
 
% \end{frame}


\begin{frame}{Evaluation: Mastermind Detection}
\begin{figure}[!t] % Use figure* for two-column format
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \includegraphics[width=\linewidth]{img/new/distribution_Out Ratio.pdf}
        \caption{Out ratio}
        \label{fig:Clustering}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \includegraphics[width=\linewidth]{img/new/distribution_Efficiency.pdf}
        \caption{Efficiency}
        \label{fig:Efficiency}
    \end{subfigure}
    \caption{(a) shows the masterminds have a higher mean out ratio and greater variability, showing a more dominant and leading role in the information spreading process. (b) shows masterminds have high efficiency, indicating accomplices are more likely to get the crowd-pump information directly from masterminds rather than their peer accomplices. }
    \label{fig:distribution}
\end{figure}
 
\end{frame}


% \begin{frame}{Discussion}
% \begin{itemize}
%     \item Our methodological framework can be easily adjusted to detect various types of financial manipulation.
%     \item Once the individuals orchestrating illegal activities are pinpointed, their public information is handed over to the appropriate authorities for further action.
%     % \item By incorporating time as a variable into the diffusion process, one may enhance detection accuracy and avoid the requirement for the event's establishment.

%     \item Limitation: 
%     \begin{enumerate}
%         \item There may be discrepancies between reality and human labelling.
%         \item The detection is time specific and token specific. Future research could aggregate the crowd-pump events from different tokens and infer the temporal attributed graphs for several tokens.
%     \end{enumerate}
% \end{itemize}


% \end{frame}

\begin{frame}{Conclusion}
    \begin{itemize}
        \item Pump-and-dump schemes in the cryptocurrency market pose a significant threat to investors. 
        \item This research pinpoints the masterminds behind such schemes and provides actionable insights for regulators.
        \item We gather the data from OSN and cryptocurrency markets, conduct topological analysis and engineer topological and market features.
        \item Subsequently, a temporal attributed graph network is developed to detect the mastermind.
        \item  By leveraging our innovative approaches, regulators can significantly enhance their oversight capabilities, reinforcing the integrity and stability of the cryptocurrency markets.
    \end{itemize}
\end{frame}



==> slides/intro.tex <==
\begin{frame}{Introduction: }
    % \begin{multicols}{2} 
        \begin{itemize}
            \item In the cryptocurrency market, a pump-and-dump is a manipulation tactic where individuals or groups artificially inflate a cryptocurrency’s price to sell it at a profit, ultimately causing significant losses for late investors.
            \item  In 2023 alone, pump-and-dump manipulators generated $241.6$ million in profit solely through decentralized exchanges, which account for only about 10\% of the total trading volume compared to centralized exchanges.
            \item Pump-and-dump schemes spreaders (masterminds and accomplices) exploit online social network (OSN)s to disseminate misleading information.
            \item Masterminds occupy upstream positions in the information diffusion process, dominating and usually controlling the entire pump-and-dump operation.
            \item This study introduces Perseus, a system that fundamentally addresses the issue of pump-and-dump schemes by tracing the masterminds within OSNs. 
            
        \end{itemize} 

\end{frame}


% \begin{frame}{Introduction:}

% \begin{itemize}
%     \item This research pioneers the systematic investigation of the pump-and-dump masterminds. Perseus detects $290$ masterminds across $322$ cryptocurrencies.
%     \item Our approach combines information from $27,365,232$ OSN messages with transaction data from $660$ cryptocurrencies, providing a multi-dimensional analysis that yields enhanced insights for regulators.
%     \item Our data pipeline processes an unprecedented dataset of cryptocurrency pump-and-dump schemes from $2,103$ channels, exceeding the scope of prior studies that examined between 50 to 700 channels.
%     \item Evaluations with real-world data have confirmed the effectiveness and efficiency of Persues, achieving a precision of 75.0\% and F1 of 75.3\% with fast training speeds and stable inference speeds.  
%     % \item \hnote{empirical results}
% \end{itemize}
% \end{frame}

\begin{frame}{Introduction:}
\begin{figure}[!t] % Use figure* to span two columns
\centering
\begin{minipage}{0.2\linewidth} % Use 49% of the text width for each figure
  \centering
  \includegraphics[height=3.5cm]{img/new/crowdpump.jpg} % Adjust height to ensure both images have the same height
  \subcaption{}
  % \caption*{(a) Crowd pump messages.}
  \label{subfig:crowd_pump message}
\end{minipage}\hfill % Fill the space between the minipages
\begin{minipage}{0.65\linewidth} % Use 49% of the text width for the second figure
  \centering
  \includegraphics[height=4.5cm]{img/new/candle_chart.png} % Adjust height to ensure both images have the same height
  \subcaption{}
  % \caption*{(b) Time pump messages.}
  \label{subfig:leverage_defi}
\end{minipage}
\caption{Crowd-pump messages are characterized by their trading pair, entry price, and target price. Crowd-pumps' impacts can last hours.}
\label{fig:crowdmarket}
\end{figure}


    
\end{frame}





==> slides/title.tex <==
\begin{frame}
    \titlepage
\end{frame}

==> storage/headers/slide-packages.tex <==
\usepackage{graphicx} % Allows including images
\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables
\usepackage{media9}
\usepackage{hyperref}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{multicol}
\hypersetup{colorlinks=true,
	linkcolor=cyan,
	citecolor=blue,
	urlcolor=green}
 
\usepackage[ruled]{algorithm2e}
\usepackage{makecell}
\usepackage{acro}
\usepackage{tabularx}
\usepackage{tikz}

==> tables/forencisc.tex <==
\begin{table*}[!h]
\centering
\footnotesize


\begin{tabularx}{\textwidth}{|c|l|c|X|c|}
\hline
\textbf{Events} & \textbf{Telegram Channels} & \textbf{Timestamps} & \textbf{Messages} & \textbf{Returns} \\ 
\hline
\textcolor{red}{$d1$} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{16/05/2019 06:50} & \textcolor{red}{\#POWR Buy zone 1360-1390 Sell zone 1490-1590-1693-1914+ Stop loss 1292} & \textcolor{red}{4.06\%} \\
   & bitcoinprofitcoach & 16/05/2019 13:01 & \#POWR Buy zone 1360-1390 Sell zone 1490-1590-1693-1914+ Stop loss 1292 & 12.27\% \\
\hline
\textcolor{red}{d2} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{08/06/2019 03:36} & \textcolor{red}{\#POWR Buy zone 1450-1495 Sell zone 1580-1644-1827-1991+ Stop loss 1300} & \textcolor{red}{6.63\%} \\
   & bitcoinprofitcoach & 08/06/2019 05:10 & \#POWR Buy zone 1360-1390 Sell zone 1490-1590-1693-1914+ Stop loss 1292 & 10.29\% \\
\hline
\textcolor{red}{d3} & bitcoinprofitcoach & 02/07/2019 18:25 & \#POWR Buy Range 1000-1040 Sell Target 1080-1125-1160-1200+ Stop loss 945 & 5.89\% \\
   & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{03/07/2019 21:03} & \textcolor{red}{\#POWR Buy zone 1040-1075 Sell zone 1140-1220-1310-1450+ Stop loss 960} & \textcolor{red}{1.17\%} \\
\hline
\textcolor{red}{d4} & bitcoinpumpgroup & 13/02/2021 04:58 & \#POWR (Binance) Buy Range : 318 - 375 Target 1: 408 Target 2: 442 Target 3: 487 Stop loss: 281@bitcoinadmin for VIP membership For Free Public Channel Link @bitcoinpumpgroup & 14.49\% \\
   & \textcolor{red}{BinanceSuperPumpSignals} & \textcolor{red}{19/02/2021 06:55} & \textcolor{red}{\#POWR (Binance) Buy zone 461-495 Sell zone 520-567-598-658-989-1200} & \textcolor{red}{13.00\%} \\
\hline
\textcolor{red}{d5} & bigpumpsignals\_official & 07/03/2021 11:46 & \#POWR (Binance) Buy zone 500-535 Sell zone 570-605-669-756+ By @crypto\_pump\_island (@APGLOBALS) & 0.15\% \\
   & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{08/03/2021 06:07} & \textcolor{red}{\#POWR (Binance) Buy zone 640-660 Sell zone 690-725-794-897+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{0.86\%} \\
\hline
\textcolor{red}{d6} & bitcoinpumpgroup & 29/03/2021 18:31 & \#POWR (Binance) Buy Range : 685 - 807 Target 1: 879 Target 2: 952 Target 3: 1049 Stop loss: 605 Contact @bitcoinadmin for VIP membership Contact For Free Public Channel Link @bitcoinpumpgroup & 10.21\% \\
   & \textcolor{red}{BinanceSuperPumpSignals} & \textcolor{red}{30/03/2021 13:43} & \textcolor{red}{\#POWR (Binance) Buy zone 867-900 Sell zone 943-978-999-1267-1678} & \textcolor{red}{7.78\%} \\
\hline
\textcolor{red}{d7} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{09/04/2021 09:12} & \textcolor{red}{\#POWR (Binance) Buy zone 875-908 Sell zone 954-1002-1098-1241+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{12.27\%} \\
   & \textcolor{red}{mega\_pump\_signals} & \textcolor{red}{09/04/2021 09:12} & \textcolor{red}{\#POWR (Binance) Buy zone 875-908 Sell zone 954-1002-1098-1241+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{12.96\%} \\
\hline
\textcolor{red}{d8} & \textcolor{red}{crypto\_pump\_island} & \textcolor{red}{27/04/2021 14:43} & \textcolor{red}{\#POWR (Binance) Buy zone 680-725 Sell zone 760-807-884-999+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{3.86\%} \\
   & bigpumpsignals\_official & 27/04/2021 14:43 & \#POWR (Binance) Buy zone 680-725 Sell zone 760-807-884-999+ By @crypto\_pump\_island (@APGLOBALS) & 3.33\% \\
\hline
\textcolor{red}{d9} & \textcolor{red}{BinanceSuperPumpSignals} & \textcolor{red}{05/02/2023 02:37} & \textcolor{red}{\#POWR/BTC (Binance) Buy zone 867-910 Sell zone 950-979-1088-1256-1954} & \textcolor{red}{10.69\%} \\
   & Binancepumpsignlas & 05/02/2023 04:15 & \#POWR/BTC (Binance) Buy zone 867-910 Sell zone 950-979-1088-1256-1954 & 1.56\% \\
\hline
\textcolor{red}{d10} & \textcolor{red}{BinanceSuperPumpSignals} & \textcolor{red}{14/10/2023 03:09} & \textcolor{red}{\#POWR/USDT (Binance) Buy zone 0.1356-0.1592 Sell zone 0.1667-0.1897-0.234-0.314 Margin 3x} & \textcolor{red}{3.60\%} \\
    & BinanceCryptoPumpSignals & 14/10/2023 03:09 & \#POWR/USDT (Binance) Buy zone 0.1356-0.1592 Sell zone 0.1667-0.1897-0.234-0.314 Margin 3x & 3.60\% \\
\hline

\textcolor{red}{d11} & \textcolor{red}{mega\_pump\_signals} & \textcolor{red}{04/01/2024 17:23} & \textcolor{red}{\#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS)} & \textcolor{red}{23.86\%} \\
    &crypto\_pump\_lsland & 04/01/2024 17:23 &\#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS) & 23.86\% \\
    & technical\_crypto\_analyst & 04/01/2024 17:23 & \#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS) & 23.86\% \\
    &cryptopumpisland1 & 04/01/2024 17:23 & \#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS) &23.86\% \\
    &BinanceTopCoin & 04/01/2024 17:23 & \#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@TraderWilliams100) & 23.86\% \\
    & crypto\_pump\_isIand\_group & 04/01/2024 17:23 & \#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS) & 23.86\% \\
    & crypto\_pump\_lsIand & 04/01/2024 17:23 & \#POWR (Binance) Buy zone 1063-1154 Sell zone 1200-1302-1382-1531+ By @crypto\_pump\_island (@APGLOBALS) & 23.86\% \\
    
\hline
d12 & Cryptotegic1 & 25/12/2023 13:15 & \#POWR/USDT Exchanges: Binance Futures Signal Type: Regular (Short) Leverage: Cross (50) Entry Targets: 0.3882 Take-Profit Targets: 1)0.3824 2)0.3785 3)0.3746 4)0.3688 5)0.3649 6)0.3591 Stop Targets: 5-10\% & 3.13\% \\
    & MCY\_TRADINGS & 25/12/2023 13:15 & \#POWR/USDT Exchanges: Binance Futures Signal Type: Regular (Short) Leverage: Cross (50) Entry Targets: 0.3882 Take-Profit Targets: 1)0.3824 2)0.3785 3)0.3746 4)0.3688 5)0.3649 6)0.3591 Stop Targets: 5-10\% & 2.77\% \\
\hline
\end{tabularx}
\caption{The crowd-pump event table outlines the channels, timing, specific messages sent, and their corresponding returns. $d_1,d_2, \ldots, d_n$ denote individual crowd pump events. Red texts highlight the crowd-pump events in which masterminds participate. Return is the maximum return achieved within three days after the announcement of the message.}
\label{tab:forencisc}

% \begin{flushleft}
% \normalsize

% \end{flushleft}

\end{table*}


==> tables/topological_features.tex <==
\begin{table}[!t]
\small
\centering
\begin{tabular}{cc}
\toprule
\textbf{Centrality Measure} & \textbf{Formula} \\
\midrule
Degree Centrality & $C_D(v) = \frac{\text{deg}(v)}{n-1}$ \\
Betweenness Centrality & $C_B(v) = \sum_{s \neq v \neq t} \frac{\sigma_{st}(v)}{\sigma_{st}}$ \\
Closeness Centrality & $C_C(v) = \frac{n-1}{\sum_{u \neq v} d(v, u)}$ \\
Clustering Coefficient & $C(v) = \frac{2T(v)}{\text{deg}(v)(\text{deg}(v)-1)}$ \\
PageRank & $PR(v) = \frac{1-d}{n} + d \sum_{u \in M(v)} \frac{PR(u)}{L(u)}$ \\
Density & $D = \frac{2m}{n(n-1)}$ \\
Effective Size & $ES = n - \frac{1}{n} \sum_{i=1}^n t_i$ \\
Efficiency & $E = 1 - \frac{1}{n^2} \sum_{i=1}^n t_i$ \\
In-Ratio & $\text{in-ratio}(v) = \frac{\text{indeg}(v)}{n}$ \\
Out-Ratio & $\text{out-ratio}(v) = \frac{\text{outdeg}(v)}{n}$ \\
\bottomrule
\end{tabular}
\caption{Table of Centrality Measures: This table outlines various centrality measures used in network analysis along with their respective formulas. Key symbols include $v$, which represents the node of interest; $\text{deg}(v)$, the degree of node $v$; $n$, the total number of nodes in the graph; $\sigma_{st}$, the total number of shortest paths from node $s$ to node $t$; $\sigma_{st}(v)$, the paths that pass through node $v$; $d(v, u)$, the shortest path distance from $v$ to other nodes $u$; $T(v)$, the number of triangles involving node $v$; $d$, the damping factor usually set at 0.85; $M(v)$, nodes that link to $v$; $L(u)$, the number of outgoing links from node $u$; $m$, the total number of edges; $t_i$, the number of ties that alter $i$ has with other alters; $\text{indeg}(v)$, the in-degree of node $v$; and $\text{outdeg}(v)$, the out-degree of node $v$.}
\label{tab:topological_features}
\end{table}

